Cauchy Completeness, Lax Epimorphisms and Effective Descent for Split Fibrations

For any suitable base category $\mathcal{V} $, we find that $\mathcal{V} $-fully faithful lax epimorphisms in $\mathcal{V} $-$\mathsf{Cat} $ are precisely those $\mathcal{V}$-functors $F \colon \mathcal{A} \to \mathcal{B}$ whose induced $\mathcal{V} $-functors $\mathsf{Cauchy} F \colon \mathsf{Cauchy} \mathcal{A} \to \mathsf{Cauchy} \mathcal{B} $ between the Cauchy completions are equivalences. For the case $\mathcal{V} = \mathsf{Set} $, this is equivalent to requiring that the induced functor $\mathsf{CAT} \left( F,\mathsf{Cat}\right) $ between the categories of split (op)fibrations is an equivalence. By reducing the study of effective descent functors with respect to the indexed category of split (op)fibrations $\mathcal{F}$ to the study of the codescent factorization, we find that these observations on fully faithful lax epimorphisms provide us with a characterization of (effective) $\mathcal{F}$-descent morphisms in the category of small categories $\mathcal{Cat}$; namely, we find that they are precisely the (effective) descent morphisms with respect to the indexed categories of discrete opfibrations -- previously studied by Sobral. We include some comments on the Beck-Chevalley condition and future work.

==> TeX/result.tex <==
\begin{theorem}
  \label{eff.desc.cauchy.comp}
  Let \( \cat D \) be a Cauchy-complete category. Every effective \(
  \Cat(-,\Set) \)-descent functor is also an effective \( \Cat(-, \cat D)
  \)-descent functor.
\end{theorem}

\begin{proof}
  For an effective \( \Cat(-,\Set) \)-descent functor \(P \colon \cat E \to
  \cat B \), consider the factorization (\ref{descent}). It follows by Theorem
  \ref{eff.desc.disc.fib} that \( \Phi^* \) is a fully faithful lax
  epimorphism, so \( \Cauchy \Phi \) is an equivalence by Lemma
  \ref{cauchy.functor}.

  Next, note that the following diagram 
  \begin{equation*}
    \begin{tikzcd}[column sep=large]
      \left[\Cauchy \Codesc P, \cat D\right] \ar[d,"\eta^*"] 
                                            \ar[r,"(\Cauchy \Phi)^*"]
        & \left[\Cauchy \cat B, \cat D\right] \ar[d,"\eta^*"] \\
      \left[\Codesc P, \cat D\right] \ar[r,"\Phi^*"] 
        & \left[\cat B, \cat D\right]
    \end{tikzcd}
  \end{equation*}
  commutes, and since \( \Cauchy \Phi \) and both \( \eta^* \) are
  equivalences, it follows that \( \Phi^* \) also is, proving our claim.
\end{proof}

\begin{lemma}
  \label{eff.desc.subcat}
  An effective \( \Cat(-,\cat D) \)-descent functor is also an effective \(
  \Cat(-,\cat C) \)-descent functor, provided there exists a fully faithful
  functor \( \cat C \to \cat D \).
\end{lemma}

\begin{proof}
  Let \( P \colon \cat E \to \cat B \) be a functor, with factorizations
  \ref{descent} for \( \cat X = \cat C,\, \cat D \). Assume we have \( F
  \colon \cat C \to \cat D \) fully faithful, and consider
  \begin{equation*}
    \begin{tikzcd}
      \Cat(\cat B, \cat C) \ar[r,"F_!"] \ar[d,"\Phi^*_{\cat C}"]
        & \Cat(\cat B, \cat D) \ar[d,"\Phi^*_{\cat D}"] \\
      \Cat(\cat E, \cat C) \ar[r,"F_!"] 
        & \Cat(\cat E, \cat D) 
    \end{tikzcd}
  \end{equation*}
  If \( P \) is an (effective) \( \Cat(-,\cat D) \)-descent functor, then we
  may conclude that \( \Phi^*_{\cat C} \) is fully faithful. To prove it is
  essentially surjective, let \( G \colon \cat E \to \cat C \) be a functor.
  Then there exists a functor \( H \colon \cat B \to \cat D \) such that \(
  H\phi_{\cat D} \iso FG \). Checking componentwise, we recover a replacement
  \( \hat H \colon \cat B \to \cat C \) such that \( \hat H \phi_{\cat C} \iso
  G \), as desired.
\end{proof}

As a corollary, we get our main result:

\begin{theorem}
  \label{main.result}
  For \( J \colon \Set \to \cat D \) fully faithful with \( \cat D \)
  Cauchy-complete, we have \( P \) of effective \( \Cat(-,\Set) \)-descent if
  and only if \( P \) is of effective \( \Cat(-,\cat D) \)-descent.
\end{theorem}
\begin{proof}
  The direct implication follows by Lemma \ref{eff.desc.subcat}, while the
  converse is a consequence of Theorem \ref{eff.desc.cauchy.comp}.
\end{proof}

